BEAMetrics: A Benchmark for Language Generation Evaluation Evaluation

Natural language processing (NLP) systems are increasingly trained to generate open-ended text rather than classifying between responses. This makes research on evaluation metrics for generated language -- functions that score system output given the context and/or human reference responses -- of critical importance. However, different metrics have different strengths and biases, and reflect human intuitions better on some tasks than others. There is currently no simple, unified way to compare, analyse or evaluate metrics across a representative set of tasks. Here, we describe the Benchmark to Evaluate Automatic Metrics (BEAMetrics), a resource to make research into new metrics itself easier to evaluate. BEAMetrics users can quickly compare existing and new metrics with human judgements across a diverse set of tasks, quality dimensions (fluency vs. coherence vs. informativeness etc), and languages. As generation experts might predict, BEAMetrics reveals stark task-dependent differences between existing metrics, and consistently poor performance on tasks with complex answer spaces or high reliance on general knowledge. While this analysis highlights a critical issue facing current research practice, BEAMetrics also contribute to its resolution by facilitating research into better metrics -- particularly those that can account for the complex interaction between context and general knowledge inherent to many modern NLP applications. BEAMetrics is available under the MIT License: https://github.com/ThomasScialom/BEAMetrics

==> draft_text.tex <==
\subsection{What is a metric?} 

In a NLG task, a model $m(x) = y_m$ must generate a phrase, sentence or passage of text $y_m$ given some input stimulus $x$.  Given such a task, an \emph{evaluation metric} is a function $f$ operating on $x_m$ and some (finite) set of `reference` phrases, sentences or passages $[r_m]$ (typically produced by human annotators) returning scalar-valued scores: $f(y_m, [r_m]) = s \in {\rm I\!R} $. A metric is therefore an evaluator function that aims to quantify the model's output given one or more examples of ideal output. 

As summarized in detail by ~\citep{sai2020survey}, metrics can be loosely categorized as either \textbf{context-dependent} or \textbf{context-independent}, depending on whether or not they consider the context $x$ as well as $y_m$ and the $[r_m]$ when computing the score $s$. Metrics can also be \textbf{trained}, if they involve a learned function, and \textbf{untrained} if they involve only non-parametric comparisons. BLEU score [REF], which considers the number of n-grams appearing in both $y_m$ and $r_m$ normalised by the length of $x_m$, is a classic example of an untrained, context-independent metric. Other metrics in this category include ROUGE [REF] and METEOR [REF]. BERTscore can be considered a trained metric, because it involves a learned embedding of both model output $y_m$ and human references $[r_m]$, but it is context-independent, as it is unaffected by $x$. Metrics like BLEURT [REF] and NUBIA incorporates a further training process, with weights fine-tuned on a set of human ratings  

Trained metrics include BERTscore, which computes similarity to human reference output 

Task-dependent or task-aware metrics?

Metrics vs. human evaluation:
- these considerations may motivate always just evaluating on humans?
